Learning Cross-Modal Affinity for Referring Video Object Segmentation Targeting Limited Samples

Referring video object segmentation (RVOS), as a supervised learning task, relies on sufficient annotated data for a given scene. However, in more realistic scenarios, only minimal annotations are available for a new scene, which poses significant challenges to existing RVOS methods. With this in mind, we propose a simple yet effective model with a newly designed cross-modal affinity (CMA) module based on a Transformer architecture. The CMA module builds multimodal affinity with a few samples, thus quickly learning new semantic information, and enabling the model to adapt to different scenarios. Since the proposed method targets limited samples for new scenes, we generalize the problem as - few-shot referring video object segmentation (FS-RVOS). To foster research in this direction, we build up a new FS-RVOS benchmark based on currently available datasets. The benchmark covers a wide range and includes multiple situations, which can maximally simulate real-world scenarios. Extensive experiments show that our model adapts well to different scenarios with only a few samples, reaching state-of-the-art performance on the benchmark. On Mini-Ref-YouTube-VOS, our model achieves an average performance of 53.1 J and 54.8 F, which are 10% better than the baselines. Furthermore, we show impressive results of 77.7 J and 74.8 F on Mini-Ref-SAIL-VOS, which are significantly better than the baselines. Code is publicly available at https://github.com/hengliusky/Few_shot_RVOS.

==> tables/table3.tex <==
\begin{tabular}{c | c | c |c}

\toprule

\multirow{1}{*}{Method} & \multirow{1}{*}{$\mathcal{J}$} & \multirow{1}{*}{$\mathcal{F}$} & \multirow{1}{*}{$\mathcal{J} \& \mathcal{F}$}  \\



\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline

\multirow{1}{*}{ReferFormer~\cite{wu2022language}} & 65.1 & 62.8 & 64\\

\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline

\multirow{1}{*}{ReferFormer*~\cite{wu2022language}} & 74.1 & 64.9 & 69.5\\

\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline

\multirow{1}{*}{Ours} & \textbf{80.9} & \textbf{77.1} & \textbf{79} \\



\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline

% \multirow{2}{*}{$\mathcal{F}$} & DAN & \multirow{2}{*}{ResNet-50} & 34.8  \\
% \multirow{2}{*}{} & Ours & \multirow{2}{*}{} & 34.8  \\

% \arrayrulecolor{white}\hline
% \arrayrulecolor{black}\hline
% \arrayrulecolor{white}\hline




\end{tabular}

==> tables/table5.tex <==
\setlength{\tabcolsep}{1.3mm}{
\begin{tabular}{p{4.2cm}<{\centering}| c | c |c | c}

\toprule

% \multirow{2}{*}{$\mathcal{J}$} & 47 & 33.5 & 38.5   \\
% \multirow{2}{*}{}  & \textbf{59.5} & \textbf{45.3} & \textbf{50.4}  \\
% \arrayrulecolor{white}\hline
% \arrayrulecolor{black}\hline
% \arrayrulecolor{white}\hline

\multirow{2}{*}{\diagbox{Unseen Class}{Method}} & \multicolumn{2}{c|}{w/o Text} & \multicolumn{2}{c}{Full Model}  \\
\cline{2-5}
\multirow{2}{*}{} & $\mathcal{J}$ & $\mathcal{F}$ & $\mathcal{J}$ & $\mathcal{F}$   \\


\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline

\multirow{1}{*}{bottle} & 77.3 & 51.6 & \textbf{82.4} & \textbf{56.3}\\

\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline

\multirow{1}{*}{coffee} & 74.7 & 64.3 & \textbf{81.3} & \textbf{71}\\

\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline

\multirow{1}{*}{lego} & 69.5 & 66.7 & \textbf{84.2} & \textbf{80.7}\\

\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline

% \multirow{1}{*}{watch} & 74.1 & 64.9 & 69.5 & 99\\

% \arrayrulecolor{white}\hline
% \arrayrulecolor{black}\hline
% \arrayrulecolor{white}\hline

\multirow{1}{*}{whisky} & 90.4 & 91.8 & \textbf{95.2} & \textbf{96.4}\\

\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline

\multirow{1}{*}{toaster} & 65 & 31.4 & \textbf{68.4} & \textbf{35.6}\\

\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline

\multirow{1}{*}{plush toy} & 69.2 & 65.8 & \textbf{78} & \textbf{68.9}\\

\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline


% \multirow{2}{*}{$\mathcal{F}$} & DAN & \multirow{2}{*}{ResNet-50} & 34.8  \\
% \multirow{2}{*}{} & Ours & \multirow{2}{*}{} & 34.8  \\

% \arrayrulecolor{white}\hline
% \arrayrulecolor{black}\hline
% \arrayrulecolor{white}\hline




\end{tabular}
}
